Variational conditional normalizing flows for computing second-order mean field control problems

Mean field control (MFC) problems have vast applications in artificial intelligence, engineering, and economics, while solving MFC problems accurately and efficiently in high-dimensional spaces remains challenging. This work introduces variational conditional normalizing flow (VCNF), a neural network-based variational algorithm for solving general MFC problems based on flow maps. Formulating MFC problems as optimal control of Fokker-Planck (FP) equations with suitable constraints and cost functionals, we use VCNF to model the Lagrangian formulation of the MFC problems. In particular, VCNF builds upon conditional normalizing flows and neural spline flows, allowing efficient calculations of the inverse push-forward maps and score functions in MFC problems. We demonstrate the effectiveness of VCNF through extensive numerical examples, including optimal transport, regularized Wasserstein proximal operators, and flow matching problems for FP equations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> old_files/2024_08_31.tex <==


In the following figure, we test several 
\begin{itemize}
    \item architecture of the flow network: number of autoregressive layer, hidden layer, hidden size of the MLP conditioner, and number of spline bins.
    \item Method to calculate the kinetic energy, but AD or finite difference.
    \item Method to evaluate the kinetic energy integration over $t$, over fixed grid or random sampled points.
\end{itemize}

\begin{table}[tb]
\caption{Evaluation of different network hyperparameters and training methods. The four number in the represents the number of autoregressive layer, the number of hidden layer in MLP conditioner, the hidden size of the MLP conditioner, and the number of bins for spline. The ``AD'' refers to calculating the kinetic energy using the auto-differentiation of the neural network while ``FD'' refers to finite difference. The grid refers to use a fixed grid of $t$ to calculate the kinetic energy integration over the time period while random refers to calculate by sampling uniformly over $[0, 1]$. The batchsize for evaluating the KL-divergence and the kinetic energy integration is set to be $2048$ and $64$ respectively. We have test that changing the batchsize as well as the ratio between the batchsize for KL loss and kinetic loss does not affect the results much. The training epoch is fixed to be $30000$ with Adam optimizer of learning rate $10^{-3}$. The speed takes into account the time of jit.}\label{table:cpu_time}
\centering
% \small
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{P{2cm} P{2cm} P{2cm} P{2cm}}
\toprule [1.5pt]
\parbox{2cm}{ Task }  & \parbox{2cm}{ \centering \# of Parameters }   &   \parbox{2cm}{ \centering Speed \\ time (iter/s)}   & \parbox{2cm}{ Accuracy } \\ \midrule[1.5pt]
{FD, random, PD}  &  2524  
 &  34.53 &  59.3\%  \\ 
{FD, random, P}  &  2524  
 &  50.63 &  1.1\%  \\ 
 {FD, grid, PD}  &  2524  
 &  35.52 &  64.2\%  \\ 
{FD, grid, P}  &  2524  
 &  57.95 &  NA  \\ 
{AD, random, PD}  &  2524  
 &  27.15 &  11.6\%  \\ 
{AD, random, P}  &  2524  
 &  42.41 &  2.3\%  \\ 
 {AD, grid, PD}  &  2524  
 &  26.76 &  NA  \\ 
{AD, grid, P}  &  2524  
 &  35.70 &  8.1\%  \\   \\ \midrule[0.5pt]
\\\bottomrule[1.5pt]
\end{tabular}
}
\end{table}

From the experiment, it is easily observed that using finite difference to calculate the kinetic energy has severe issue. This may be caused by the network directly hacked the sample points along the time trajectory. Namely, as the velocity is approximated by finite difference, the optimization forces the network to minimize the finite difference along the collocation point, meaning that most adjacent pair of the collocation point corresponds to the same mapping and transition between the initial and terminal conditions may happen at very small time interval. Notice that even if we dynamically sample the collocation point uniformly in $[0,1]$ during each epoch the problem is not resolved. \JX{However, this may also happen to the AD method and our explanation does not distinguish between these two.}

==> old_files/method_with_time_varying_parameters.tex <==
\section{Time-dependent parameter approach}
We consider a general Mean field control problem
\begin{align}
  \min_{\{\rho(\cdot, t)\}_{0\leq t \leq T}, \{\textbf{v}(\cdot, t)\}_{0\leq t \leq T}} & \left\{ \int_0^T \int_\Omega L(x, \textbf{v}(x, t), \rho_t)~\rho_t(x)~dx ~dt + \mathcal G(\rho_T) \right\}  \label{MFcontrol}\\
  \textrm{Subject to } & \partial_t{\rho(x,t)} + \nabla\cdot(\rho \textbf{v}) = D \Delta \rho, \quad \rho_0 = \rho_{\textrm{init}}.\nonumber
\end{align}
The Lagrangian could take the form
\begin{equation}
  L(x, v, \rho) = \frac{\|v\|^2}{2} + V(x) + \eta(\rho(x)),  \label{separate L}
\end{equation}
in which case, $L$ is decomposed as the sum of the kinetic energy, potential energy, and interaction energy.

Given a parameter space $\Theta$, suppose we consider pushforwad map $f_\theta(\cdot):Z\rightarrow \Omega$ with each $\theta \in \Theta$, we consider time dependent parameter $\{\theta_t\}_{0\leq t\leq T}$. We use the trajectory $\{f_{\theta_t}(\cdot)_\# p\}\subset \mathcal{P}(\Omega)$ to approximate the optimal trajectory of the mean-field control problem \eqref{MFcontrol}.

Notice that when the diffusion coefficient $D=0$, the vector field $\textbf{v}(\cdot, t)$ that drives the particle $f_{\theta_t}(\textbf{z})$ is $\frac{\partial f_{\theta_t}(\textbf{z})}{\partial \theta} \dot\theta_t$. And the distribution of the particle $f_{\theta_t}(\textbf{z})$ is $f_{\theta_t}(\cdot)_\# p$. Plugging them into \eqref{MFcontrol}, we come up with an analogy of the original mean-field control problem on $\Theta$, which can be formulated as:
\begin{align*}
  \min_{\{\theta_t\} ~ \textrm{with }\theta_0 = \theta_\textrm{init}, \{\dot\theta_t\}}  \left\{\int_0^T L^\Theta(\theta_t, \dot\theta_t) ~dt + G^\Theta(\theta_T)  \right\}
\end{align*}
Here we need to find $\theta_\textrm{init}$ such that $f_{\theta_\textrm{init}}(\cdot)_\# p = \rho_{\textrm{init}}.$

Furthermore, 
\begin{equation*}
  L^\Theta(\theta, \dot\theta) = \int_Z L(f_\theta(z), \frac{\partial f_\theta(z)}{\partial \theta}\dot\theta, f_{\theta}(\cdot)_\# p ) ~p(z) dz.
\end{equation*}
\begin{equation*}
  G^\Theta(\theta) = \mathcal G(f_\theta(\cdot)_\# p).
\end{equation*}

In the case of separated Lagrangian \eqref{separate L}, 
\[ L^\Theta(\theta, \dot\theta) = \frac12 \dot\theta^\top G(\theta) \dot\theta + \int_Z V(f_\theta(z))~dp(z) + \int_Z \eta(\rho_\theta(f_\theta(z)))~dp(z), \quad (\rho_\theta \triangleq f_\theta(\cdot)_\# p.) \]
where $G(\theta)$ denotes the Wasserstein metric tensor on $\Theta$,
\[ G(\theta) = \int_Z \frac{\partial f_\theta(z)}{\partial \theta}^\top \frac{\partial f_\theta(z)}{\partial \theta} ~dp(z). \]

By introducing the adjoint variable $\{p_t\}$ for $\frac{d\theta_t}{dt} = \dot\theta_t$, we obtain the following saddle point problem
\begin{align*}
  \max_{\{p\}}~\min_{\{\theta\}, \{\dot\theta\}}~~ \left\{ \int_0^T -\frac{d p_t}{dt}^\top \theta_t -( \dot\theta_t^\top p_t - L^\Theta(\theta_t, \dot\theta_t)) ~ dt + G^\Theta(\theta_T) + \theta_T^\top p_T - \theta_\textrm{init}^\top p_0 \right\}.
\end{align*}
This can be simplified to (By minimizing over $\{\dot\theta\}$, and the optimal value of $\dot\theta$ is $\dot\theta = \frac{\partial L^\Theta(\theta, \cdot)}{\partial v}^{-1}(p_t)$.)
\begin{align*}
  \max_{\{p\}}~\min_{\{\theta\}}~~ \left\{ \int_0^T -\frac{d p_t}{dt}^\top \theta_t -H^\Theta(\theta_t, p_t) ~ dt + G^\Theta(\theta_T) + \theta_T^\top p_T - \theta_\textrm{init}^\top p_0 \right\},
\end{align*}
where we define 
\[ H^\Theta(\theta, p) = \sup_{v\in\mathcal T_\theta \Theta} ~ \{v^\top p - L^\Theta(\theta, v)\}.\]
The Pontryagin principle (KKT) associated with the control problem yields (the first line is due to $\frac{d \theta_t}{dt}=\dot\theta = \frac{\partial L^\Theta(\theta, \cdot)}{\partial v}^{-1}(p_t) = \frac{\partial H^\Theta(\theta_t, p_t)}{\partial p}$)
\begin{align*}
  \frac{d \theta_t}{dt} &  =  \frac{\partial H^\Theta(\theta_t, p_t)}{\partial p}, \quad \theta_0 = \theta_\textrm{init};\\
  \frac{d p_t}{dt} & = -\frac{\partial H^\Theta(\theta_t, p_t) }{\partial \theta_t}, \quad p_T = -\partial_\theta G^\Theta(\theta_T).
\end{align*}


\subsection{Derivation of HJD equation on parameter space}

For the potential MFG, one can derive its associated Hamilton-Jacobi equation on density manifold (HJD equation). Then the MFG system becomes the characteristic line of the HJD equation. 

We consider the control problem
\begin{align*}
  \min_{\{\rho_s\}_0^T} \left\{ \int_0^T \mathcal L(\rho_s, \dot\rho_s)~ds + \mathcal G(\rho_T) \right\}
\end{align*}
The Lagrangian $\mathcal L$ here only depends on data $(\rho, \dot\rho)$ from the probability density manifold. In the case of \eqref{MFcontrol} with $D=0$, the running cost depends further on velocity field $\textbf{v}$, which carrys more information than $\dot\rho$. But one can still formulate \eqref{MFcontrol} in the form of $\mathcal L(\rho, \dot\rho)$. One can verify that 
\[ \mathcal L(\rho, \dot\rho) = 
\begin{cases}
    \min_{\textbf{v}} ~ \int_\Omega L(x, \textbf{v}(x), \rho)\rho(x)~dx\\
    \textrm{subject to } ~ -\nabla\cdot(\rho\textbf{v}(x)) = \dot\rho.
\end{cases} \]
The Lagrange multiplier method yields
\[ \mathcal L(\rho, \dot\rho) = \int_\Omega L(x, (\nabla_vL(x, \cdot, \rho))^{-1}(\nabla\Phi(x)), \rho) \rho(x)~dx, \]
where $\Phi$ solves
\[ -\nabla\cdot(\rho (\nabla_vL(x, \cdot, \rho))^{-1}(\nabla\Phi(x))) = \dot\rho(x). \]

We denote the value functional
\[ \mathcal U(\rho, t) = \min_{\{\rho_s\}_t^T, ~\rho_t = \rho} \left\{ \int_t^T \mathcal L(\rho_s, \dot\rho_s) ~ds + \mathcal G(\rho_T) \right\}. \]
Now we (formally) derive the HJD equation via Bellman principle
\begin{align*}
  \mathcal U(\rho, t) & = \min_{\rho_{t+h}} \left\{ \int_t^{t+h} \mathcal L(\rho_s, \dot\rho_s)~ds + \mathcal U(\rho_{t+h}, t+h) \right\} \\
  & \approx \min_{\rho_{t+h}} \left\{ \mathcal L(\rho, \frac{\rho_{t+h} - \rho}{h}) \cdot h + \mathcal U(\rho_{t+h}, t+h) \right\}  .
\end{align*}
Then we have
\begin{align*}
  \frac{\mathcal U(\rho, t) - \mathcal U(\rho, t+h)}{h} = &  \min_{\rho_{t+h}} \left\{ \mathcal L(\rho, \frac{\rho_{t+h} - \rho}{h}) + \frac{\mathcal U(\rho_{t+h}, t+h) - \mathcal U(\rho, t+h)}{h} \right\}\\
  \approx & \min_{D_h \rho_{t}} \left\{ \mathcal L (\rho, D_h\rho_t) + \Bigg\langle \frac{\delta \mathcal U(\rho, t+h)}{\delta \rho}, D_h\rho_t 
  \Bigg\rangle \right\} , 
\end{align*}
where we denote $D_h \rho_t = \frac{\rho_{t+h} - \rho}{h}$.

We further denote the Legendre transform of $\mathcal L$ as
\begin{equation*}
  \mathcal H(\rho, \Phi) \triangleq \max_{\dot\rho\in\mathcal T_\rho\mathcal P} \left\{ \langle \Phi, \dot\rho \rangle - \mathcal L(\rho, \dot\rho)  \right\}.
\end{equation*}

By taking the variation w.r.t. $D_h\rho_t$ of the above minimization problem, we know the optimal moving direction is 
\[ D_h \rho_t = (\frac{\delta}{\delta \dot\rho} \mathcal L(\rho, \cdot))^{-1} (- \frac{\delta \mathcal U(\rho, t+h)}{\delta \rho}) = \frac{\delta}{\delta \Phi} \mathcal H(\rho, - \frac{\delta \mathcal U(\rho, t+h)}{\delta \rho}). \] 


Then the above equation yields
\begin{equation*}
  \frac{\mathcal U(\rho, t) - \mathcal U(\rho, t+h)}{h} = - \mathcal H(\rho, -\frac{\delta \mathcal U(\rho, t+h)}{\delta \rho}).
\end{equation*}
We send $h\rightarrow 0$, which yields the Hamilton-Jacobi equation on the probability density manifold $\mathcal P$ (HJD).
\begin{equation}
  -\frac{\partial }{\partial t} \mathcal U(\rho, t) + \mathcal H(\rho, -\frac{\delta \mathcal U(\rho, t)}{\delta \rho}) = 0, \quad \mathcal U(\rho, T) = \mathcal G(\rho). \label{HJDE}
\end{equation}

Then the MFC system 
\begin{align*}
  & \frac{\partial \rho}{\partial t} = \frac{\delta}{\delta \Phi} \mathcal H(\rho, - \frac{\delta \mathcal U(\rho, t)}{\delta \rho})\\
  & \frac{\partial \Phi}{\partial t} = - \frac{\delta}{\delta \rho} \mathcal H(\rho, - \frac{\delta \mathcal U(\rho, t)}{\delta \rho}),
\end{align*}
can be treated as the characteristic of the HJD equation \eqref{HJDE}.



Now, for the Mean-Field control problem projected on the parameter manifold $\Theta$ of a generative model
\begin{align*}
  \min_{\{\theta_t\} ~ \textrm{with }\theta_0 = \theta_\textrm{init}, \{\dot\theta_t\}}  \left\{\int_0^T L^\Theta(\theta_t, \dot\theta_t) ~dt + G^\Theta(\theta_T)  \right\},
\end{align*}
we can introduce the value functional
\[ \mathcal U^\Theta(\theta, t) = \min_{\{\theta_t\}_t^T ~ \textrm{with }\theta_t = \theta, \{\dot\theta_t\}}  \left\{\int_t^T L^\Theta(\theta_t, \dot\theta_t) ~dt + G^\Theta(\theta_T)  \right\}. \]

By using the similar technique, one can derive the associated HJD equation on $\Theta$ as
\begin{equation} 
  -\frac{\partial}{\partial t}\mathcal U^\Theta (\theta, t) + H^\Theta(\theta, -\nabla_\theta \mathcal U^\Theta(\theta, t))=0, \quad \mathcal U^\Theta(\theta, T) = G^\Theta(\theta) = \mathcal G(\rho_{\theta}).  \label{PHJD} 
\end{equation}


By setting $p_t = \nabla_\theta \mathcal U^\Theta(\theta, t)$, one can verify that the characteristic 
\[ \dot\theta = - \nabla_\theta \mathcal U^\Theta(\theta_t, t), \]
reduces to   
\begin{align*}
  \frac{d \theta_t}{dt} &  =  \frac{\partial H^\Theta(\theta_t, p_t)}{\partial p}, \quad \theta_0 = \theta_\textrm{init};\\
  \frac{d p_t}{dt} & = -\frac{\partial H^\Theta(\theta_t, p_t) }{\partial \theta_t}, \quad p_T = -\partial_\theta G^\Theta(\theta_T).
\end{align*}

\wc{In potential MFGs, the master equation is an evolution equation for $u( \theta, t)=\nabla_{\theta}\mathcal{U}^{\Theta}(\theta, t)$. 
}


\wc{Can we also derive the projected dynamics and master equations for non-potential mean field games? }




The MFG is formulated as follows.

Fix the time-dependent probability distribution $\{\mu_t\}_0^T$. Consider the optimal solution to the following stochastic control problem
\begin{align*}
    & \min_{\{v_t\}_{0\leq t \leq T}}~\mathbb{E}\left[ \int_0^T K(\boldsymbol{X}_t, v_t(\boldsymbol{X}_t)) + F(\boldsymbol{X}_t, \mu_t)~dt + G(\boldsymbol{X}_T, \mu_T)\right],\\
    & \textrm{s.t. } d\boldsymbol{X}_t = v_t(\boldsymbol{X}_t)~dt + \sqrt{2}d\boldsymbol{B}_t, \quad \boldsymbol{X}_0\sim\rho_0.
\end{align*}
Let us denote the optimal solution to this control problem as $\{v^*_t\}$, and its associated trajectory $\{\boldsymbol{X}_t\}$ as $\{\boldsymbol{X}^*_t\}$. Recall that $\{\boldsymbol{X}^*_t$\} depends on $\{\mu_t\}$. Our goal is to find $\{\mu_t\}_0^T$ such that $\textrm{Law}(\boldsymbol{X}^*_t) = \mu_t$ for $t\in[0, T]$.

One can reformulate the above MFG as follows.

Fix the time-dependent probability distribution $\{\mu_t\}_0^T$. Consider the optimal solution to the following density control problem
\begin{align*}
    & \min_{\{v_t\}_{0\leq t \leq T}}~\left[ \int_0^T \int_\Omega (K(x, v_t(x)) + F(x, \mu_t)) \rho_t(x)~dx~dt + \int_\Omega G(x, \mu_T)\rho_T(x)~dx\right],\\
    & \textrm{s.t. } \frac{\partial \rho_t}{\partial t} + \nabla\cdot(\rho_t v_t) = \Delta \rho_t\quad \textrm{with initial condition } \rho_0 .
\end{align*}
Denote the optimal solution to this problem as $\{ \rho^*_t \}$. We want to find $\{\mu_t\}$ such that $\rho^*_t = \mu_t$ for $t\in[0, T]$.

We want to project this MFG onto the parameter space of the Neural network. By picking 
a reference probability measure $p$, we approximate $\rho_t$ by $T_{\theta_t \sharp}\lambda$, here $\{T_\theta\}_{\theta\in\Theta}, T_\theta:Z\rightarrow \Omega$ is a family of parametrized pushforward maps, and $\{\theta_t\}_{0\leq t\leq T}\subset\Theta$ denotes a trajectory in the parameter space. We further assume that $\Theta\subset\mathbb{R}^m$.
 
Recall that the FP equation $\frac{\partial \rho_t}{\partial t} + \nabla\cdot(\rho_t v_t) = \Delta \rho_t$ can be reformulated as
\[ \frac{\partial \rho_t}{\partial t} + \nabla\cdot(\rho_t(v_t - \nabla\log\rho_t)) = 0.    \]
And the continuity equation associated with $\{T_{\theta_t}\}$ is
\[\frac{\partial \rho_{\theta_t}}{\partial t} + \nabla\cdot(\rho_{\theta_t} ~ \frac{\partial T_{\theta_t}}{\partial \theta}\circ T_{\theta_t}^{-1}(\cdot) \dot \theta) = 0. \]
Then $v_t(\cdot)$ can be approximated by
\begin{equation*}
  v_{\theta_t}(\cdot) = \frac{\partial T_{\theta_t}}{\partial \theta} \circ T_{\theta_t}^{-1}(\cdot) ~ \dot\theta + \nabla \log\rho_{\theta_t}(\cdot).
\end{equation*}

Then the density control problem projected on $\Theta$ can be formulated as:

\begin{align}
    \min_{\{\theta_t\}_{0\leq t \leq T}}~\left\{ \int_0^T \underbrace{\int_Z (K(T_{\theta_t}(z), v_{ \theta_t }(T_{\theta_t}(z))) + F(T_{\theta_t}(z), \mu_t)) \lambda(z)~dz}_{\textrm{denote as }\mathcal L^\Theta(\theta_t, \dot\theta, \mu_t)}~dt + \underbrace{\int_\Omega G(T_{\theta_T}(z), \mu_T)\lambda(z)~dz}_{\textrm{denote as } \mathcal G^\Theta(\theta_T, \mu_T)}\right\}. \label{MFG NN}
\end{align}
Now we define the Hamiltonian
\begin{align*}
  \mathcal H^\Theta(\theta, p, \mu) & = \max_{\zeta \in \mathbb{R}^m } ~ \{\zeta^\top p - \mathcal L^\Theta(\theta, \zeta, \mu)\} \\ 
  & = \max_{\zeta \in \mathbb{R}^m } ~ \{ \zeta^\top p - \int_Z  K(T_{\theta}(z), \frac{\partial T_{\theta_t}(z)}{\partial \theta}  ~  \zeta + \nabla \log\rho_{\theta_t}(T_{\theta_t}(z)))~d\lambda(z)   \} \\
  & \quad  - \int_Z F(T_\theta(z), \mu )~d\lambda(z) - \int_Z G(T_\theta(z), \mu) ~d\lambda(z).
\end{align*}
The optimal solution of \eqref{MFG NN} is given by the following dynamic
\begin{align}
    \dot \theta_t = & \frac{\partial}{\partial p}\mathcal H^\Theta(\theta_t, p_t, \mu_t), ~ \textrm{with initial condition }\theta_0 \textrm{ s.t. } T_{\theta_0\sharp}p \approx \rho_0, \label{MFG NN 1}\\
     \dot p_t = & - \frac{\partial}{\partial \theta}\mathcal H^\Theta(\theta_t, p_t, \mu_t)  , ~  p_T = - \nabla_\theta \mathcal G^\Theta(\theta_T, \mu_T),  \label{MFG NN 2}
\end{align}
Recall that at the Nash equilibrium of the MFG, we have $\rho_t = \mu_t$. This indicates that we can replace $\mu_t$ in \eqref{MFG NN 1} and \eqref{MFG NN 2} by $T_{\theta_t \sharp}  \lambda$ and directly solve for $\{\theta_t\}_0^T.$

That is, we compute for $\{\theta_t\}_0^T$ as the solution of the following equation system
\begin{align}
    \dot \theta_t = & \frac{\partial}{\partial p}\mathcal H^\Theta(\theta_t, p_t, T_{\theta_t\sharp} \lambda), ~ \textrm{with initial condition }\theta_0 \textrm{ s.t. } T_{\theta_0\sharp} \lambda \approx \rho_0, \label{MFG NN Nash equ 1}\\
     \dot p_t = & - \frac{\partial}{\partial \theta}\mathcal H^\Theta(\theta_t, p_t, T_{\theta_t \sharp } \lambda)  , ~  p_T = - \partial_\theta \mathcal G^\Theta(\theta_T, T_{\theta_t\sharp} \lambda),  \label{MFG NN Nash equ 2}
\end{align}


\wc{Can we formulate an algorithm for the neural mean field games? 
Instead of gradient descent. We need a Montone inclusion algorithm. We summarize these into one algorithm.}

\wc{Check examples with $$F(x,\rho)=\int W(x,y)\rho(y)dy,$$
where $W(x,y)\neq W(y,x)$.}

\wc{Derive the master equation on neural networks \cite{WA}. See related approaches in \cite{GLL}.}

==> old_files/numerical_example_Mo.tex <==
\section{Additional numerical Examples}
In this section we provide some concrete examples.\mz{TODO: Unify the notations in the end.}

\subsection{Wasserstein Proximal Operator with double well potential}
This example is from \cite{li2023kernel}. \mz{Be careful that the $\beta$ in \cite{li2023kernel} equals to our $\frac{1}{\beta}$ in the first example.} We can set $V$ to be a double well potential, given by
$V(x) = \frac14 (x-c_1)^2 (x-c_2)^2$. \mz{You can also test other potential you like.} The explicit solution is given by Proposition 4 and 5 in \cite{li2023kernel}, including the density $\rho$ and the solution to the HJB equation $\Phi$. The optimal velocity field is $v^* = \nabla \Phi$, with $\Phi$ given by equation (11) in \cite{li2023kernel}.

\begin{proposition}[Kernel solutions]
The following solutions hold.
\begin{equation}\label{rho}
\rho(t,x)=\frac{1}{{(4\pi\frac{1}{\beta}\frac{t(T-t)}{T}})^{\frac{d}{2}}}\int_{\mathbb{R}^d}\int_{\mathbb{R}^d}\frac{e^{-\frac{\beta}{2}(V(z)+\frac{\|x-z\|^2}{2(T-t)}+\frac{\|x-y\|^2}{2t})}}{\int_{\mathbb{R}^d}e^{-\frac{\beta}{2}(V(\tilde y)+\frac{\|y-\tilde y\|^2}{2T})}\rd \tilde y}\rho(0,y) \rd y\rd z,
\end{equation}
and 
\begin{equation}\label{Phi}
\Phi(t,x)=\frac{2}{\beta} \log\Big(\int_{\mathbb{R}^d}\frac{1}{(\frac{4\pi}{\beta} (T-t))^{\frac{d}{2}}}e^{-\frac{\beta}{2}(V(y)+\frac{\|x-y\|^2}{2(T-t)})}\rd y\Big).
\end{equation}
In particular, 
\begin{equation*}
\rho(T,x)=\int_{\mathbb{R}^d}K(x,y, \beta, T, V)\rho(0,y)\rd y,
\end{equation*}
where $K\colon \mathbb{R}^d\times\mathbb{R}^d\times \mathbb{R}_+\times \mathbb{R}_+\times C^1(\mathbb{R}^d)\rightarrow\mathbb{R}$ is the kernel function 
\begin{equation}\label{kernel}
K(x,y,\beta, T,V):=\frac{e^{-\frac{\beta}{2}(V(x)+\frac{\|x-y\|^2}{2T})}}{\int_{\mathbb{R}^d}e^{-\frac{\beta}{2}(V(z)+\frac{\|z-y\|^2}{2T})}\rd z}.
\end{equation}

\end{proposition}


\subsection{Reversible time diffusion}
This example comes from \cite{zhang2023mean} Theorem 7. The difference between this example and the first one is that we have an additional drift $f$. The objective is 

$$\begin{aligned} & \inf_{v, \rho}\left\{-\int_{\mathbb{R}^d} \log \Pi(x) \rho(T,x) \rd  x+\int_0^T \int_{\mathbb{R}^d}\left(\frac{1}{2}|v(t,x)|^2-\nabla \cdot f(t,x)\right) \rho(t,x) \rd  x \rd  t\right\} \\ & \text { s.t. } \frac{\partial \rho(t,x)}{\partial t}+\nabla \cdot[(f(t,x)+\sigma(t) v(t,x)) \rho(t,x)]=\frac{1}{2} \sigma(t)^2 \Delta \rho(t,x) \\ & \rho(0,x)=\rho_0(x)\end{aligned}$$
with controlled dynamics
$$\rd  x_t=[f(t,x_t)+\sigma(t) v(t,x_t)] \, \rd  t+\sigma(t) \, \rd  W(t)$$
The solution of the mean-field game satisfies the optimality conditions.
\begin{equation*}
\left\{\begin{array}{l}
-\dfrac{\partial U}{\partial t}-f^{\top} \nabla U+\frac{1}{2}|\sigma \nabla U|^2+\nabla \cdot f=\frac{\sigma^2}{2} \Delta U \\
\dfrac{\partial \rho}{\partial t}+\nabla \cdot\left(\left(f-\sigma^2 \nabla U\right) \rho\right)=\frac{\sigma^2}{2} \Delta \rho \\
U(T,x)=-\log \Pi(x), \rho(0,x)=\rho_0(x) .
\end{array}\right.
\end{equation*}
where the optimal velocity field has the representation formula
$$v^*(t,x) = -\sigma(t) \nabla U(t,x).$$ 

We can consider the specific example where $f(t,x) = -x$, $\sigma(t)=1$ and $\Pi(x)$ is a centered Gaussian $N(0,C*I_d)$. In this case, the solution to the HJB equation is of the form $U(t,x) = \frac12 \Gamma_2(t) |x|^2 + \Gamma_0(t)$ where
\begin{equation}
\Gamma_2(t) = \dfrac{2}{1 + ce^{2t}}
\end{equation}
and
\begin{equation}
\partial_t \Gamma_0(t) + \frac12 \Gamma_2(t) = 0.    
\end{equation}
\mz{This is obtained by plugging $U(t,x) = \frac12 \Gamma_2(t) |x|^2 + \Gamma_0(t)$ into the HJB equation. Need check.}
The terminal condition of $\Gamma_2(t)$ and $\Gamma_0(t)$ is given by $\Pi(x)$. For example, if we take $\Pi \sim N(0,I_d)$, then $-\log\Pi(x) = \frac12 |x|^2 +\frac{d}{2} \log(2\pi)$. So, $\Gamma_2(T) = 1$ and $\Gamma_0(T) = \frac{d}{2} \log(2\pi)$. In this case,
\begin{equation}
\Gamma_2(t) = \dfrac{2}{1 + e^{2(t-T)}}.
\end{equation}
It seems we do not need $\Gamma_0(t)$. The optimal stochastic trajectory is hence given by
\begin{equation}
\rd x_t = - \parentheses{ \dfrac{2}{1 + e^{2(t-T)}} + 1} x_t \,\rd t + \rd W_t.
\end{equation}
This makes $x_t$ remain a centered Gaussian $N(0,\Sigma(t))$ as long as $x_0 \sim N(0,\Sigma_0)$ is a centered Gaussian. $\Sigma(t)$ satisfies
\begin{equation}
\pt \Sigma(t) = -2 \parentheses{ \dfrac{2}{1 + e^{2(t-T)}} + 1} \Sigma(t) + I_d \quad\quad \Sigma(0) = \Sigma_0
\end{equation}
 \mz{We are able to obtain an explicit solution, but it looks complicated. Maybe it is better to solve the ODE numerically to obtain a reference solution.}
Let $T=1$, then the solution is \mz{might be wrong, I may make mistakes}
\begin{equation}
\Sigma(t) = \mathrm{e}^{-6t} \parentheses{\dfrac{1+\mathrm{e}^{2(t-1)}}{1+\mathrm{e}^{-2}}}^2 \sqbra{\Sigma_0 + \int_0^t \dfrac{\mathrm{e}^{6s}}{(1+\mathrm{e}^{2(s-1)})^2} \,\rd s \, I_d}
\end{equation}
where
\begin{align*}
& \int_0^t \dfrac{\mathrm{e}^{6s}}{(1+\mathrm{e}^{2(s-1)})^2} \,\rd s  = -\frac{\mathrm{e}^{2t + 6} \ln\left(\mathrm{e}^{2t} + \mathrm{e}^{2}\right)}{\mathrm{e}^{2t} + \mathrm{e}^{2}} - \frac{\mathrm{e}^{8} \ln\left(\mathrm{e}^{2t} + \mathrm{e}^{2}\right)}{\mathrm{e}^{2t} + \mathrm{e}^{2}} + \frac{\mathrm{e}^{4t + 4}}{2 \left(\mathrm{e}^{2t} + \mathrm{e}^{2}\right)} + \frac{\mathrm{e}^{2t + 6}}{2 \left(\mathrm{e}^{2t} + \mathrm{e}^{2}\right)} \\
& - \frac{\mathrm{e}^{8}}{2 \left(\mathrm{e}^{2t} + \mathrm{e}^{2}\right)} + \frac{\mathrm{e}^{8} \ln\left(\mathrm{e}^{2} + 1\right)}{\mathrm{e}^{2} + 1} + \frac{\mathrm{e}^{6} \ln\left(\mathrm{e}^{2} + 1\right)}{\mathrm{e}^{2} + 1} + \frac{\mathrm{e}^{8}}{2 \left(\mathrm{e}^{2} + 1\right)} - \frac{\mathrm{e}^{6}}{2 \left(\mathrm{e}^{2} + 1\right)} - \frac{\mathrm{e}^{4}}{2 \left(\mathrm{e}^{2} + 1\right)}
\end{align*}


==> old_files/numerics.tex <==
\section{Potential algorithm}
We propose the following algorithm to calculate the Wasserstein geodesic between $\rho_0$ and $\rho_1$. Using $\forall t \in [0,1], f_{\theta}(\mfz; t): Z \rightarrow \Omega$ to parametrize the geodesic $\rho_t, t\in[0, 1]$
such that $\rho_t = f_{\theta}(\cdot; t)_\#p$ where $p$ can be any base measure, i.e. Gaussian. We use a neural network to parametrize $f_{\theta}$ that takes both $z, t$ as input and $x$ as output. Then, the loss function can be written as 
\begin{equation}
  \begin{aligned}
    L(\theta) = & \ \int_0^1 \int_{Z}\p_t f_{\theta}(z; t)^T \p_t f_{\theta}(z; t) p(z)dz + d(\rho_0, f_{\theta}(\cdot; 0)_\#p) +  d(\rho_1, f_{\theta}(\cdot; 1)_\#p)      \\
    = & \ \frac{1}{t_N N}\sum_{i=1}^{t_N} \sum_{j=1}^N \lb \p_t f_{\theta}(z_j; t_I)^T \p_t f_{\theta}(z_j; t_i) \rb + d(\rho_0, \frac{1}{N}\sum_{j=1}^N \delta_{f_{\theta}(z_j; 0)}) \\
    & \ + d(\rho_1, \frac{1}{N}\sum_{j=1}^N \delta_{f_{\theta}(z_j; 1)}).
  \end{aligned}
\end{equation}

The other option is to consider
\begin{equation}
  \begin{aligned}
    L(\theta) = & \ \int_0^1 \int_{Z}\p_t f_{\theta}(z; t)^T \p_t f_{\theta}(z; t) p(z)dz  +  \int V(x) f_\theta(\cdot;1)_{\#}p dx      \\
    = & \ \frac{1}{t_N N}\sum_{i=1}^{t_N} \sum_{j=1}^N \lb \p_t f_{\theta}(z_j; t_I)^T \p_t f_{\theta}(z_j; t_i) \rb  + \frac{1}{N}\sum_{j=1}^NV(f_\theta(z_j;1)).
  \end{aligned}
\end{equation}
Here $V(x)=\frac{\|x\|^2}{2}$ and $f_{\theta}(z;0)=z$. 

\wc{Two choices: 
\begin{itemize}
\item 
\begin{equation*}
 \int_0^1\int_Z \partial_t f_\theta^{T}\partial_tf_\theta   p_r(z)dzdt\approx 1/N*\sum_{k=1}^N\frac{1}{\Delta t^2}( f_{\theta^{k+1}}-f_{\theta^k})^2\Delta t, 
\end{equation*}
where $\theta^{k}=\theta(t^k)$, $t^k=k*\Delta t$, $\Delta t$ is a stepsize. 
\item
\begin{equation*}
 \int_0^1\dot \theta^{T} G(\theta)\dot \theta dt\approx \sum_{k=1}^N(\frac{\theta^{k+1}-\theta^k}{\Delta t})^TG(\theta^k)(\frac{\theta^{k+1}-\theta^k}{\Delta t})\Delta t=\sum_{k=1}^NF( \theta^k,\theta^{k+1}),
\end{equation*}
where 
\begin{equation*}
 F(\theta^{k},\theta^{k+1})=(\frac{\theta^{k+1}-\theta^k}{\Delta t})^TG(\theta^k)(\frac{\theta^{k+1}-\theta^k}{\Delta t})\Delta t,
\end{equation*}
and 
\begin{equation*}
   G(\theta )_{ij}=E_{z\sim p} \Big[\partial_{\theta_i}f^T\partial_{\theta_j}f\Big]. 
\end{equation*}
Here
\begin{equation*}
  \nabla_{\theta_k}F(\theta^k,\theta^{k+1})= ....
\end{equation*}

The other idea is that we parameterize $\theta(t)$ by a neural network and directly train time-dependent networks. 
\end{itemize}
\wc{After the successful choices of methods, we may think about the natural gradient (precondition gradient type) methods in solving the proposed projected control problem. }
}


In the last line, we use Monte Carlo to sample from the base distribution $p$ to estimate the value of the loss function.
And $d(\cdot, \cdot)$ is chosen by some distance measure such as KL-divergence and MMD which is easy to evaluate. The term $\p_t f_{\theta}(z_j; t_I)^T \p_t f_{\theta}(z_j; t_i)$ can be evaluated by 
back-propagating through neural networks

\JX{This is more or less similar to the work \cite{doi:10.1073/pnas.2024713118}, better to come up with a novel idea. Their generator network is also not linear over $t$. 

We also need to compare with results in Rongjie Lai's Bridging Mean-Field Games and Normalizing Flows with
Trajectory Regularization. }




\subsection{Comparison to other formulations}
\subsubsection{Density parametrization}
\subsubsection{Velocity parametrization}
This approach is more similar to our approach on mapping parametrization. The difference is that velocity field is directly parametrized as
\begin{equation}
    NN_{\phi}(x, t) = \nabla_t f_{\theta}(x, t),
\end{equation}
instead of the mapping function. There are following advantanges and disadvantages for this approach:
\begin{itemize}
    \item \textbf{Advantage:} the velocity is directly modeled by neural network hence during optimization only the first order information needs to be calculate, which makes the kinetic part computationally easier.
    \item \textbf{Disadvantage 1:} the boundary condition is hard to encode as one needs to integrate along the whole trajectory starting from initial distribution to obtain the probability distribution at terminal time. Therefore the KL-divergence term in the objective function is hard to handle. This also makes the sampling extremely inefficient comparing to our approach.
    \item \textbf{Disadvantage 2:} \JX{although reversible map is not necessary at current stage, would that be a issue to guarantee the reversibility here?}
\end{itemize}

\newpage


\section{Numerical experiments}
Numerical experiments are presented in this section to illustrate the performance of our algorithm.

\subsection{Conditional normalizing flow}
We propose to use the conditional normalizing flow (CNF) introduced by \cite{winkler2019learning} for our experiments. Different from original normalizing flow for probabilistic inference, CNF adds extra parameters called condition into the network which is the time in our case. Let us briefly mention the architecture of the network. Fix a reference measure $p_{\text{r}}(\mfz)$ over the latent variable $\mfz$ which is standard Gaussian in our case. The normalizing flow models the target distribution $p(\mfx)$ via a chain of invertible transformation based on rational quadratic spline as follows
\begin{equation}\label{eq:flow}
    p_{\text{r}}(\mfz) \overset{f_{\theta, t}}{\rightleftharpoons} p(\mfx, t).
\end{equation}
Notice that both the forward mapping $f_{\theta, t}$ and inverse mapping $f_{\theta, t}^{-1}$ can be evaluated and differentiated, $\theta$ denote all the trainable parameters of the network model, and $t$ denotes the time index which is also an input of the flow network. 
Notice the difference between our model and models belong to the family of neural ODE \cite{chen2018neural} is that: in their model, mappings corresponding to different time step is composited together to form the final mapping while in our model they are not composited, share the same network parameters but the different time index. 
% Mathematically, the model can be written as 
% \begin{equation}
%     \mfz_{k+1} = f_{\theta, t_k}(\mfz_{k}) = \text{NN}_{\theta}(\mfz_{k}, t_k), \quad \mfx = \mfz_{n+1}.
% \end{equation}
Under this framework, we can sample from $p(\cdot, T)$ and any intermediate distribution $p(\cdot, t)$ by sampling from $p_{\text{r}}$ then push forward. Therefore, any objective function that can be written as the expectation over some intermediate distribution can be evaluated efficiently via Monte Carlo. The kinetic energy is related to the time derivative, which can be calculated via auto-differentiation over the network as the time $t$ is also the input. Although the kinetic energy at time step $t$ should be integrated over the intermediate measure $p_t$, it is more efficient to use change of variable formula to integrate over the reference distribution $p_{\text{r}}$ as
\begin{equation}
    E_{\text{kin}}(t) = \mbE_{\mfz \sim p_{\text{r}}}\norml \p_t \text{NN}_{\theta}(\mfz, t) \normr_2^2.
\end{equation}
The last one is the score function of the target distribution at time $t$, i.e.
\begin{equation}
    s(\mfx, t) = \nabla_{\mfx}\log p(\mfx, t).
\end{equation}
Given any $\mfx$, as the inverse mapping $f_{\theta, t}^{-1}$ is available and auto-differentiable, we can calclate the corresponding latent vector $\mfz$ by 
\begin{equation}
    \mfz = f_{\theta, t}^{-1}(\mfx) = \text{NN}_{\theta}^{-1}(\mfx, t).
\end{equation}
Then, the log probability $\log p(\mfx, t)$ can be evaluated via Monge-Ampere equation as
\begin{equation}
    \log p(\mfx, t) = \log p_{\text{r}}(\mfz) - \log \lv J_{f_{\theta, t}}(\mfz) \rv = \log p_{\text{r}}(\text{NN}_{\theta}^{-1}(\mfx, t)) - \log \lv J_{f_{\theta, t}}(\text{NN}_{\theta}^{-1}(\mfx, t)) \rv,
\end{equation}
where $\lv J_{f_{\theta, t}} \rv$ denote the Jacobian of the mapping $f_{\theta, t}$. Notice that all the components above can be auto-differentiated and thus score function can be calculated directly by (auto) differeentiating $\log p(\mfx, t)$ over $\mfx$.
\JX{We can add more discussions on formulating different building blocks in our setting if later numerical examples contain.}

\wc{Some tricks to compute or approximate $f^{-1}$ are needed. }

\textbf{Gaussian example}

We first perform sanity check to see whether conditional normalizing flow has the ability to fit two Gaussians in 2D with:
\begin{equation}
   \rho_{\theta}(\cdot|t=0) \sim \mcN\lp\begin{pmatrix}
       -1 \\ -1
   \end{pmatrix}, \mfI \rp, \quad \rho_{\theta}(\cdot|t=1) \sim \mcN\lp\begin{pmatrix}
       3 \\ 3
   \end{pmatrix}, \mfI \rp.
\end{equation}
The result is shown in \cref{fig:CNF}, where the left figure is sampling from $t=0,1$ at the initialization while the right one is sampling from the optimized conditional normalizing flow.
The loss function is the summation of the two KL-divergence at the two distributions:
\begin{equation}
  \begin{aligned}
    L(\theta) = d(\rho_0, \frac{1}{N}\sum_{j=1}^N \delta_{f_{\theta}(z_j; 0)}) + d(\rho_1, \frac{1}{N}\sum_{j=1}^N \delta_{f_{\theta}(z_j; 1)}).
  \end{aligned}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=.6\textwidth]{fig/CNF.pdf}  
    \caption{Fitting a conditional normalizing flow for two Gaussian.}
    \label{fig:CNF}
\end{figure}

\textbf{Gaussian mixture example}

\subsection{Wassertein distance}

\textbf{1D example}


\textbf{2D example}
For solving the Wasserstein geodesic which is a constrained optimization problem, we relax the constrained and include it into the loss function as
\begin{equation}
  \begin{aligned}
    L(\theta) = & \ \int_0^1 \int_{Z}\p_t f_{\theta}(z; t)^T \p_t f_{\theta}(z; t) p(z)dz + d(\rho_0, f_{\theta}(\cdot; 0)_\#p) +  d(\rho_1, f_{\theta}(\cdot; 1)_\#p)      \\
    = & \ \frac{\lambda}{t_N N}\sum_{i=1}^{t_N} \sum_{j=1}^N \lb \p_t f_{\theta}(z_j; t_I)^T \p_t f_{\theta}(z_j; t_i) \rb + d(\rho_0, \frac{1}{N}\sum_{j=1}^N \delta_{f_{\theta}(z_j; 0)}) \\
    & \ + d(\rho_1, \frac{1}{N}\sum_{j=1}^N \delta_{f_{\theta}(z_j; 1)}).
  \end{aligned}
\end{equation}
Notice that we introduce a tunable parameter $\lambda$ to the loss function which controls the ratio between the KL-divergence loss and the kinetic energy. For $\lambda=0.1$, the optimization results are illustrated in \cref{fig:geo-1}.
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{fig/weight0.1.pdf}
        \caption{Distributions at $t=0,1$}
    \end{subfigure}
    \hfill % adds horizontal space between the figures
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{fig/weight0.1_traj.pdf}
        \caption{Interpolation between two distributions}
    \end{subfigure}
    \caption{}
    \label{fig:geo-1}
\end{figure}
While if we shrink the parameter $\lambda$ to $0.01$, it is easy to observe in \cref{fig:geo-2} that two distributions at the end points are captured better.
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{fig/weight0.01.pdf}
        \caption{Distributions at $t=0,1$}
    \end{subfigure}
    \hfill % adds horizontal space between the figures
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{fig/weight0.01_traj.pdf}
        \caption{Interpolation between two distributions}
    \end{subfigure}
    \caption{}
    \label{fig:geo-2}
\end{figure}
The evolution velocity field at each time step is also shown in \cref{fig:traj0.01}
\begin{figure}[ht]
    \centering
        \includegraphics[width=\textwidth]{fig/weight0.01_velo.pdf}
        \caption{Velocity field along the transport. Kinetic energy $12.07$.}
    \label{fig:traj0.01}
\end{figure}

\subsection{Linear quadratic control} 
The objective is defined by 
\begin{equation}\label{eq:lqr-objective}
\inf_v \int_0^T \int_{\RR^d} \parentheses{\frac12\abs{v(t,x)}^2 + \gamma\parentheses{\frac12 \rho(t,x) - \rho^*(t,x)}} \rho(t,x) \,\rd x \,\rd t + \int_{\RR^d} V(x) \rho(T,x) \,\rd x
\end{equation}
subject to the dynamic
\begin{equation}\label{eq:ODE_x_v}
\pt x_t = v(t,x_t) - \frac1\beta \nabla_x \log \rho(t,x_t),
\end{equation}
with initial distribution $\rho_0 \sim N(0, 2(T+1) I_d / \beta)$.  In this example, the term with coefficient $\gamma$  is intentionally introduced to increase the difficulty of the problem. The FP-HJB system governing this problem is
\begin{equation*}
\left\{\begin{aligned}
&\pt\rho(t,x) + \nabla_x\cdot \parentheses{\rho(t,x) \nabla_x\phi(t,x)}=\frac1\beta \Delta_x \rho(t,x),\\
&\pt\phi(t,x) + \frac12 \abs{\nabla_x \phi(t,x)}^2 + \frac1\beta \Delta_x\phi(t,x) = \gamma\parentheses{\rho(t,x) - \rho^*(t,x)},\\
& \rho(0,x)=\rho_0(x),\quad \phi(T,x)=-V(x)=-|x|^2/2. 
\end{aligned}\right.
\end{equation*}
Here, $\rho^*$ is the true solution with the optimal trajectory, given by
\begin{equation*}
\rho^*(t,x) = \parentheses{4\pi (T-t+1)/\beta}^{-\frac{d}{2}} \exp\parentheses{-\dfrac{\beta\abs{x}^2}{4 (T-t+1)}}.
\end{equation*}
The solution to the HJB equation is 
\begin{equation*}
\phi(t,x) = \frac1\beta d\log\frac{1}{T-t+1}-\frac{\abs{x}^2}{2(T-t+1)}.
\end{equation*}
The optimal velocity is $v^* = \nabla \phi$.
\mz{you can set $\gamma=0$ for simplicity, then the problem becomes Wasserstein proximal operator problem. In this case, we have explicit solution for non-Gaussian example, using kernel formula.}
Given the close form solution, we can obtain the exact value of the objective function for $\beta = 1$ as
\begin{equation}
    \begin{aligned}
        & \ \int_0^T \int_{\RR^d} \frac12\abs{v^*(t,x)}^2 \rho^*(t,x) \,\rd x \,\rd t + \int_{\RR^d} V(x) \rho^*(T,x) \,\rd x     \\
        = & \ \int_0^T \int_{\RR^d} \frac{|x|^2}{2(T-t+1)^2} \rho^*(t,x) \,\rd x \,\rd t + \int_{\RR^d} \frac12 |x|^2 \rho^*(T,x) \,\rd x   \\
        = & \ \int_0^T \frac{\,\rd t}{(T-t+1)} + 1 = \log 2 + 1.
    \end{aligned}
\end{equation}

Next, we discuss how to calculate the objective function \cref{eq:lqr-objective} under our network model. For simplicity, we
\begin{equation}
  \begin{aligned}
    L(\theta) = & \ \int_0^1 \int_{Z}\p_t f_{\theta}(z; t)^T \p_t f_{\theta}(z; t) p(z)dz + \lambda d(\rho_0, f_{\theta}(\cdot; 0)_\#p) + \mbE_{x \sim f_{\theta}(\cdot; 1)_\#p)}[V(x)]      \\
    = & \ \frac{1}{t_N N_k}\sum_{i=1}^{t_N} \sum_{j=1}^{N_k} \norml \p_t f_{\theta}(z_j^{k}; t_i) + \frac{1}{\beta}\nabla_x \log p(f_{\theta}(z_j^{k}; t_i), t_i) \normr^2      \\
    & \ + \lambda d(\rho_0, \frac{1}{N_0}\sum_{j=1}^{N_0} \delta_{f_{\theta}(z_j^{(0)}; 0)}) + \frac{1}{N_1}\sum_{j=1}^{N_1} V(f_{\theta}(z_j^{(1)}; 1)),
  \end{aligned}
\end{equation}
where $N_0, N_1, N_k$ stand for the batch size for the initial condition loss, potential loss, and kinetic energy loss of the objective function.
\subsubsection{Tunning regularization constant}
As our flow model \cref{eq:flow} has free initial distribution, we add constraint to force the initial condition of the LQR example.


\begin{figure}[ht]
% \vspace{-0.1in}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{fig/0.00_lambda10.pdf}
        \includegraphics[width=\textwidth]{fig/0.20_lambda10.pdf}
        \includegraphics[width=\textwidth]{fig/0.40_lambda10.pdf}
        \includegraphics[width=\textwidth]{fig/0.60_lambda10.pdf}
        \includegraphics[width=\textwidth]{fig/0.80_lambda10.pdf}
        \includegraphics[width=\textwidth]{fig/1.00_lambda10.pdf}
        \includegraphics[width=\textwidth]{fig/mfg_kin_lambda10.pdf}
        \caption{$\lambda$ = 10, 100k epochs}
        \label{fig:sub1}
    \end{subfigure}
    % \hfill % adds horizontal space between the figures
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{fig/0.00_lambda20.pdf}
        \includegraphics[width=\textwidth]{fig/0.20_lambda20.pdf}
        \includegraphics[width=\textwidth]{fig/0.40_lambda20.pdf}
        \includegraphics[width=\textwidth]{fig/0.60_lambda20.pdf}
        \includegraphics[width=\textwidth]{fig/0.80_lambda20.pdf}
        \includegraphics[width=\textwidth]{fig/1.00_lambda20.pdf}
        \includegraphics[width=\textwidth]{fig/mfg_kin_lambda20.pdf}
        \caption{$\lambda$ = 20, 100k epochs}
        \label{fig:sub2}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{fig/0.00_lambda50.pdf}
        \includegraphics[width=\textwidth]{fig/0.20_lambda50.pdf}
        \includegraphics[width=\textwidth]{fig/0.40_lambda50.pdf}
        \includegraphics[width=\textwidth]{fig/0.60_lambda50.pdf}
        \includegraphics[width=\textwidth]{fig/0.80_lambda50.pdf}
        \includegraphics[width=\textwidth]{fig/1.00_lambda50.pdf}
        \includegraphics[width=\textwidth]{fig/mfg_kin_lambda50.pdf}
        \caption{$\lambda$ = 50, 100k epochs}
        \label{fig:sub3}
    \end{subfigure}
    \caption{We compare the numerical results using different regularization parameters $\lambda$ to enforce the initial condition. All three cases (column) are performed over the same network architecture with one auto-regressive layer, all MLP conditioners have one hidden layer with dimension $16$, $20$ bins for each spline. \JX{Maybe we could state these default setting somewhere.} From left to right, the $\lambda$ is increasing, meaning a strong penalty over the initial condition. As a result, we conclude that the compute velocity $\dot{x}$ is more accurate at the beginning, i.e. $t=0.00$ for larger $\lambda$. On the other hand, a strong penalization on the initial condition will also influences the original minimization problem to solve the LQR, making it less accurate. Viewing from the figure, we observe that the compute velocity is less accurate at later time step for larger $\lambda$, which can also be concluded from the trends of the error $\left\| \dot{x} - \dot{x}_* \right\|^2$.} 
    \label{fig:tunning-reg}
    \vspace{0.0in}
\end{figure}

\subsection{Optimal transport with obstacle}
\XZ{We consider transporting $\rho_0$ to $\rho_1$ with the added constraint that the population tend to avoid some area during the transportation. This is commonly considered in mean field control problems. Specifically, we consider a potential $V(x)$ in \eqref{separate L} of the form 
$$
V(x) = \gamma \max \left\{-x^T \begin{pmatrix}
    5&0\\
    0&-1
\end{pmatrix}x -0.1,0\right\} \,,
$$
where $\gamma>0$ (e.g. $\gamma=5$). An additional congestion loss could also be considered to encourage the agents to spread apart. In this case, we choose $\eta(\rho)$ in \eqref{separate L} to be an interaction kernel: 
$$
\eta(\rho)(y) = (W*\rho)(y) = \int_{\Omega} W(y-x) \rho(y) dy = \int_{\Omega} \frac{1}{\|y-x\|^2 + 1}\rho(y) dy  \,, 
$$

\subsection{Acceleration control}
Instead of minimizing the action, which is the time integral of the kinetic energy, we consider minimizing the time integral of the (2-norm of) acceleration vector considered by \cite{craig2024blob}. In details, we change the $\|v\|^2/2$ term in \eqref{separate L} into $\|a\|^2/2$ where $a(t) = \ddot x(t)=\dot v(t)$ is the acceleration vector. Note that our Lagrangian now also depends on $a$. In terms of implementation, this amounts to simply changing $\partial_t f_{\theta}(z,t)$ into $\partial_{tt} f_{\theta}(z,t)$. 



\subsection{Update on the 2D experiments}
There are lots of training hyperparameters which can be tuned for a better training routine. We list them all here and discuss how to investigate this systematically.

\subsubsection{Expressivity of the flow model}
In this subsection, we test that whether the flow model we used is able to

\begin{table}[tb]
\caption{Density fitting of conditional NF. All the optimizations perform 20000 iterations and all the criterions are calculated using Monte Carlo sampling. Moreover, we evaluate the error of the transport map against the optimal transport map in the appendix.}\label{table:density-fitting}
\centering
% \small
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{P{4cm} P{2cm} P{2cm} P{2cm} P{2cm} }
\toprule [1.5pt]
\parbox{4cm}{ Density }   &   \parbox{2cm}{ \centering $\mathrm{D}_{\mathrm{KL}}(\widehat{\rho}_0\|\rho_0)$}   & \parbox{2cm}{ \centering $\mathrm{D}_{\mathrm{KL}}(\widehat{\rho}_1\|\rho_1)$ } & \parbox{2cm}{\centering  $\norml \widehat{\rho}_0 - \rho_0 \normr_2^2$ }  
& \parbox{2cm}{ \centering $\norml \widehat{\rho}_1 - \rho_1 \normr_2^2$ }\\ \midrule[1.5pt]
\parbox{4cm}{$N(\begin{pmatrix}
    0\\0
\end{pmatrix},\mathbf{I}), N(\begin{pmatrix}
    1\\1
\end{pmatrix},\mathbf{I})$} 
 &  1.1045E-1 &  8.5007E-2 &  4.7840E-4 & 3.6900e-4    \\ \midrule[0.5pt]
\parbox{4cm}{$N(\begin{pmatrix}
    -1\\-1
\end{pmatrix},\mathbf{I}), N(\begin{pmatrix}
    1\\1
\end{pmatrix},\mathbf{I})$} 
 &  1.4593E-1 &  1.2852E-1 &  3.1067E-4 & 3.2195E-4    \\ \midrule[0.5pt]
\parbox{4cm}{$N(\begin{pmatrix}
    -2\\-2
\end{pmatrix},\mathbf{I}),N(\begin{pmatrix}
    2\\2
\end{pmatrix},\mathbf{I})$} 
 &  2.5594E-2 &  2.4006E-2 &  1.7808E-5 & 1.2438E-5    \\ \midrule[0.5pt]
 \parbox{4cm}{$N(\begin{pmatrix}
    -3\\-3
\end{pmatrix},\mathbf{I}), N(\begin{pmatrix}
    3\\3
\end{pmatrix},\mathbf{I})$} 
 &  3.7176E-3 &  6.4874E-3 &  1.2566E-5 & 3.2728E-5    \\ \midrule[0.5pt]
 \parbox{4cm}{$N(\begin{pmatrix}
    -5\\-5
\end{pmatrix},\mathbf{I}),N(\begin{pmatrix}
    5\\5
\end{pmatrix},\mathbf{I})$} 
 &  1.6610E-3 &  4.9648E-3 &  7.3586E-6 & 2.3387E-5    \\ \midrule[0.5pt]
\parbox{5cm}{$N(\begin{pmatrix}
    -5\\-5
\end{pmatrix},\mathbf{I}),N(\begin{pmatrix}
    5\\5
\end{pmatrix},0.25\mathbf{I})$} 
 &  1.9334E-3 &  3.4815E-3  &  1.2149E-5  & 3.6665E-4    \\ \midrule[0.5pt]
\parbox{5cm}{$N(\begin{pmatrix}
    -5\\-5
\end{pmatrix},\mathbf{I}), N(\begin{pmatrix}
    5\\5
\end{pmatrix},0.09\mathbf{I})$} 
 &  1.7207E-3 &  1.8334E-3  &  8.3851E-6  &1.1591E-3    \\ \midrule[0.5pt]
 \parbox{5cm}{$N(\begin{pmatrix}
    -5\\-5
\end{pmatrix},\mathbf{I}), N(\begin{pmatrix}
    5\\5
\end{pmatrix},0.04\mathbf{I})$} 
 &  NaN &  NaN &  NaN  & NaN    \\ \midrule[0.5pt]
\\\bottomrule[1.5pt]
\end{tabular}
}
\end{table}


\textbf{Loss function}
\begin{itemize}
    \item Use KL or MSE loss to enforce the initial condition.
    \item The hyperparameter $\lambda$ to tune between the error of constraint penalty and kinetic energy. Wuchen suggests using the gradient descent ascent to optimize the $\lambda$ simultaneously.
    \item To calculate the kinetic energy, we need to evaluate the integration related to it. There are two approaches: calculating using the Monte Carlo sampling, calculating using several collocation points over the uniform grid.
    \item For the Gaussian model, 
\end{itemize}

\textbf{Network architecture}
\begin{itemize}
    \item The width of the MLP conditioner.
    \item The number of AR layers.
\end{itemize}

}

\begin{itemize}
    \item Use finite difference to calculate the velocity is faster, but not effective.
    \item Number of autoregressive layer is the most important.
    \item The training is not very stable.
    \item Primal-dual is not very effective.
\end{itemize}
